SGSimEval: A Comprehensive Multifaceted and Similarity-Enhanced Benchmark for Automatic Survey Generation Systems

The growing interest in automatic survey generation (ASG), a task that traditionally required considerable time and effort, has been spurred by recent advances in large language models (LLMs). With advancements in retrieval-augmented generation (RAG) and the rising popularity of multi-agent systems (MASs), synthesizing academic surveys using LLMs has become a viable approach, thereby elevating the need for robust evaluation methods in this domain. However, existing evaluation methods suffer from several limitations, including biased metrics, a lack of human preference, and an over-reliance on LLMs-as-judges. To address these challenges, we propose SGSimEval, a comprehensive benchmark for Survey Generation with Similarity-Enhanced Evaluation that evaluates automatic survey generation systems by integrating assessments of the outline, content, and references, and also combines LLM-based scoring with quantitative metrics to provide a multifaceted evaluation framework. In SGSimEval, we also introduce human preference metrics that emphasize both inherent quality and similarity to humans. Extensive experiments reveal that current ASG systems demonstrate human-comparable superiority in outline generation, while showing significant room for improvement in content and reference generation, and our evaluation metrics maintain strong consistency with human assessments.

==> table.tex <==
\begin{table}[ht!]
    \centering
    \scriptsize
    \setlength{\tabcolsep}{2pt}
    \renewcommand{\arraystretch}{1.2}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l
        |l
        |c c
        |c c c c c c
        |c c 
        }
    \hline
    \multirow{2}{*}{\textbf{System}} 
    & \multirow{2}{*}{\textbf{Domain}}
    & \multicolumn{2}{c|}{\textbf{Outline}} 
    & \multicolumn{6}{c|}{\textbf{Content}} 
    & \multicolumn{2}{c}{\textbf{Reference}} \\
    
    & 
    & \makecell{Quality}
    & \makecell{Structure} 
    
    & \makecell{Coverage} 
    & \makecell{Structure} 
    & \makecell{Relevance} 
    & \makecell{Language} 
    & \makecell{Criticalness} 
    & \makecell{Faithfulness}
    
    & \makecell{Quality} 
    & \makecell{Supportiveness}\\
    
    
    \toprule
    \textbf{AutoSurvey}
    & \textit{SGEval} &  &  &  &  &  &  &  &  & \\
    & \textit{SGEval-Sim} &  &  &  &  &  &  &  &  & \\
    \midrule
    \textbf{InteractiveSurvey}
    & \textit{SGEval} &  &  &  &  &  &  &  &  & \\
    & \textit{SGEval-Sim} &  &  &  &  &  &  &  &  & \\
    \midrule
    \textbf{LLMxMapReduce}
    & \textit{SGEval}&  &  &  &  &  &  &  &  & \\
    & \textit{SGEval-Sim} &  &  &  &  &  &  &  &  & \\
    \midrule
    \textbf{SurveyForge}
    & \textit{SGEval}&  &  &  &  &  &  &  &  & \\
    & \textit{SGEval-Sim} &  &  &  &  &  &  &  &  & \\
    \midrule
    \textbf{SurveyX}
    & \textit{SGEval} &  &  &  &  &  &  &  &  & \\
    & \textit{SGEval-Sim} &  &  &  &  &  &  &  &  & \\
    \midrule
    \textbf{Human}
    & \textit{SGEval} &  &  &  &  &  &  &  &  & \\
    \bottomrule
    \end{tabular}
    }
    \caption{Hierarchical Evaluation Metrics for Survey Generation Systems Across Different Models. (Now with two-level headers: groups and detailed metrics.)}
    \label{tab:experiment_results}
\end{table}

\begin{table}[ht!]
    \centering
    \scriptsize
    \setlength{\tabcolsep}{2pt}
    \renewcommand{\arraystretch}{1.2}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|l|c|c}
    \toprule
    \textbf{System} & \textbf{Outline} & \textbf{Content} & \textbf{Reference} \\
    \hline
    \textbf{AutoSurvey}         & 0.70 & 0.20 & 0.20 \\
    \hline
    \textbf{InteractiveSurvey}  & 0.39 & 0.23 & 0.13 \\
    \hline
    \textbf{LLMxMapReduce}      & 0.74 & 0.37 & 0.02 \\
    \hline
    \textbf{SurveyForge}        & 0.50 & 0.00 & 0.70 \\
    \hline
    \textbf{SurveyX}            & 0.62 & 0.07 & 0.21 \\
    \bottomrule
    \end{tabular}
    }
    \caption{Simplified Evaluation Metrics for Survey Generation Systems Across Different Models.}
    \label{tab:experiment_results_similarity}
\end{table}

==> tables/criteria.tex <==
\begin{table}[th]
    \centering
    \tiny 
    \caption{Content Quality Criteria.}
    \label{table:criteria}
    \begin{tabularx}{\linewidth}{@{}lX@{}} % Use tabularx with \linewidth; X column for wrapping text
        \toprule
        \textbf{Criteria} & \textbf{Scores} \\
        \midrule
        \textbf{Coverage} & 
        \textit{Score 1}: The survey has very limited coverage, only touching on a small portion of the topic and lacking discussion on key areas. \\
        & \textit{Score 2}: The survey covers some parts of the topic but has noticeable omissions, with significant areas either underrepresented or missing. \\
        & \textit{Score 3}: The survey is generally comprehensive in coverage but still misses a few key points that are not fully discussed. \\
        & \textit{Score 4}: The survey covers most key areas of the topic comprehensively, with only very minor topics left out. \\
        & \textit{Score 5}: The survey comprehensively covers all key and peripheral topics, providing detailed discussions and extensive information. \\
        \midrule
        \textbf{Structure} & 
        \textit{Score 1}: The survey lacks logic, with no clear connections between sections, making it difficult to understand the overall framework. \\
        & \textit{Score 2}: The survey has weak logical flow with some content arranged in a disordered or unreasonable manner. \\
        & \textit{Score 3}: The survey has a generally reasonable logical structure, with most content arranged orderly, though some links and transitions could be improved such as repeated subsections. \\
        & \textit{Score 4}: The survey has good logical consistency, with content well arranged and natural transitions, only slightly rigid in a few parts. \\
        & \textit{Score 5}: The survey is tightly structured and logically clear, with all sections and content arranged most reasonably, and transitions between adjacent sections smooth without redundancy. \\
        \midrule
        \textbf{Relevance} & 
        \textit{Score 1}: The content is outdated or unrelated to the field it purports to review, offering no alignment with the topic. \\
        & \textit{Score 2}: The survey is somewhat on topic but with several digressions; the core subject is evident but not consistently adhered to. \\
        & \textit{Score 3}: The survey is generally on topic, despite a few unrelated details. \\
        & \textit{Score 4}: The survey is mostly on topic and focused; the narrative has a consistent relevance to the core subject with infrequent digressions. \\
        & \textit{Score 5}: The survey is exceptionally focused and entirely on topic; the article is tightly centered on the subject, with every piece of information contributing to a comprehensive understanding of the topic. \\
        \midrule
        \textbf{Language} & 
        \textit{Score 1}: The language is highly informal, contains frequent grammatical errors, imprecise terminology, and numerous colloquial expressions. The writing lacks academic tone and professionalism. \\
        & \textit{Score 2}: The writing style is somewhat informal, with several grammatical errors or ambiguous expressions. Academic terminology is inconsistently used. \\
        & \textit{Score 3}: The language is mostly formal and generally clear, with only occasional minor grammatical issues or slightly informal phrasing. \\
        & \textit{Score 4}: The language is clear, formal, and mostly error-free, with only rare lapses in academic tone or minor imprecisions. \\
        & \textit{Score 5}: The writing is exemplary in academic formality and clarity, using precise terminology throughout, flawless grammar, and a consistently scholarly tone. \\
        \midrule
        \textbf{Criticalness} & 
        \textit{Score 1}: The survey lacks critical analysis and fails to identify gaps, weaknesses, or areas for improvement. Offers no original insights and does not propose any meaningful future research directions. \\
        & \textit{Score 2}: The survey provides only superficial critique, with limited identification of weaknesses. Original insights are minimal and future directions are vague or generic. \\
        & \textit{Score 3}: The survey demonstrates moderate critical analysis, identifying some gaps or weaknesses. Offers some original perspectives and suggests future directions, though they may lack depth or specificity. \\
        & \textit{Score 4}: The survey presents a strong critique, clearly identifying significant gaps and weaknesses, and proposes well-justified future research directions. Provides some novel insights, though a few aspects could be further developed. \\
        & \textit{Score 5}: The survey excels in critical analysis, incisively evaluating methodologies, results, and assumptions. Provides highly original insights and proposes clear, actionable, and innovative future research directions, all rigorously justified. \\
        \midrule
        \textbf{Outline} & 
        \textit{Score 1}: The outline is chaotic or confusing, with unclear relationships and significant structural gaps. Section titles are vague, repetitive, or lack logical flow. \\
        & \textit{Score 2}: The outline shows basic attempts at organization but contains multiple misplaced or poorly grouped sections. The progression is unclear or disjointed. Section titles are sometimes ambiguous. \\
        & \textit{Score 3}: The outline demonstrates a generally reasonable structure, with some minor misalignments or grouping issues. Most section titles are clear, and topic coverage is mostly logical. \\
        & \textit{Score 4}: The outline is well-structured, with clearly grouped section titles and a coherent progression of topics. Minor issues may exist but do not significantly affect readability or understanding. \\
        & \textit{Score 5}: The outline is exceptionally clear, logically organized, and easy to follow. Section titles are concise and informative, and the structure fully represents the topic's breadth and depth. \\
        \midrule
        \textbf{Reference} & 
        \textit{Score 1}: Most references (over 60\%) are irrelevant or only marginally related to the topic. \\
        & \textit{Score 2}: A significant portion (40-60\%) of references are not closely related to the topic. \\
        & \textit{Score 3}: Some references (20-40\%) are not relevant to the topic, but the majority are appropriate. \\
        & \textit{Score 4}: A small number (5-20\%) of references are not well aligned, but most are relevant. \\
        & \textit{Score 5}: Nearly all references (over 95\%) are relevant and directly related to the topic. \\
        \bottomrule
    \end{tabularx}
\end{table}
